A Learning-Based Framework for Line-Spectra Super-resolution

We propose a learning-based approach for estimating the spectrum of a multisinusoidal signal from a finite number of samples. A neural-network is trained to approximate the spectra of such signals on simulated data. The proposed methodology is very flexible: adapting to different signal and noise models only requires modifying the training data accordingly. Numerical experiments show that the approach performs competitively with classical methods designed for additive Gaussian noise at a range of noise levels, and is also effective in the presence of impulsive noise.

==> sr_figure.tex <==
\begin{figure}[tp]
\hspace{-0.4cm}
\begin{tabular}{ >{\centering\arraybackslash}m{0.07\linewidth} >{\centering\arraybackslash}m{0.28\linewidth} >{\centering\arraybackslash}m{0.28\linewidth} >{\centering\arraybackslash}m{0.28\linewidth}}%{  c ccc }
& \footnotesize{Infinite samples} \vspace{0.1cm} & $N = 40$ \vspace{0.1cm} & $ N = 20$ \vspace{0.1cm} \\
\footnotesize{Signal} &  
\begin{tikzpicture}[scale=0.55]
\begin{axis}[xmin=-2.5,xmax=53,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,},xlabel=Time]
\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
\addplot[only marks,very thick,blue] file {dat_files/spectral_superres/sines_samples_long_3.dat};
\addplot[black] coordinates {(-10,0) (100,0)};
\end{axis}
\end{tikzpicture} 
&
\begin{tikzpicture}[scale=0.55]
\begin{axis}[xmin=-2.5,xmax=53,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,},xlabel=Time]
\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
\addplot[only marks,very thick,blue] file {dat_files/spectral_superres/sines_samples_long_2.dat};
\addplot[black] coordinates {(-10,0) (100,0)};
\end{axis}
\end{tikzpicture} 
&
\begin{tikzpicture}[scale=0.55]
\begin{axis}[xmin=-2.5,xmax=53,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,},xlabel=Time]
\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
\addplot[only marks,very thick,blue] file {dat_files/spectral_superres/sines_samples_long.dat};
\addplot[black] coordinates {(-10,0) (100,0)};
\end{axis}
\end{tikzpicture} 
\\
\footnotesize{Spectrum} & % \hspace{0.3cm}
\begin{tikzpicture}[scale=0.55]
\begin{axis}[yticklabels={,,},xmin=0.1,xmax=0.5,width=0.6\textwidth, height=0.4\textwidth,xlabel=Frequency] 
\addplot+[ycomb,mark=none,very thick,violet] file {dat_files/spectral_superres/sines_spectrum.dat};
\addplot[black] coordinates {(0,0) (0.5,0)};
\end{axis}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=0.55]
\begin{axis}[yticklabels={,,},width=0.6\textwidth, height=0.4\textwidth,xmin=0.1,xmax=0.5,xlabel=Frequency] %
\addplot+[ycomb,mark=none,very thick,red,dashed] file {dat_files/spectral_superres/sines_spectrum.dat};
\addplot[very thick,violet] file {dat_files/spectral_superres/sines_lowres_long_2.dat};
\addplot[black] coordinates {(0,0) (0.5,0)};
\end{axis}
\end{tikzpicture} 
&
\begin{tikzpicture}[scale=0.55]
\begin{axis}[yticklabels={,,},width=0.6\textwidth, height=0.4\textwidth,xmin=0.1,xmax=0.5,xlabel=Frequency] %
\addplot+[ycomb,mark=none,very thick,red,dashed] file {dat_files/spectral_superres/sines_spectrum.dat};
\addplot[very thick,violet] file {dat_files/spectral_superres/sines_lowres_long.dat};
\addplot[black] coordinates {(0,0) (0.5,0)};
\end{axis}
\end{tikzpicture}
\end{tabular}
\caption{Illustration of the spectral super-resolution problem. A multisinusoidal signal following Eq.~\eqref{eq:model} (dashed blue) and its Nyquist-rate samples (blue) are depicted on the top row. The resolution of the spectrum (purple) depends on the number of samples $N$ used to compute the discrete-time Fourier transform (bottom row). The signal is real-valued, so its spectrum is even; only half of it is shown.}
\label{fig:spectral_sr}
\end{figure}

%\begin{figure}[tp]
%\begin{center}
%\begin{tabular}{  >{\centering\arraybackslash}m{0.39\linewidth} >{\centering\arraybackslash}m{0.45\linewidth} }
%  Periodogram & Data \\ \\
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[ticks=none,width=0.6\textwidth, height=0.45\textwidth,xmin=0.1,xmax=0.5] %
%\addplot+[ycomb,mark=none,very thick,red,dashed] file {dat_files/spectral_superres/sines_spectrum.dat};
%\addplot[very thick,violet] file {dat_files/spectral_superres/sines_lowres.dat};
%\addplot[black] coordinates {(0,0) (0.5,0)};
%\end{axis}
%\end{tikzpicture} 
%&
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[xmin=-2.5,xmax=12.5,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,}]
%\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
%\addplot[only marks, thick,blue] file {dat_files/spectral_superres/sines_samples.dat};
%\addplot[black] coordinates {(-10,0) (50,0)};
%\end{axis}
%\end{tikzpicture} 
%\\
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[ticks=none,width=0.6\textwidth, height=0.45\textwidth,xmin=0.1,xmax=0.5] %
%\addplot+[ycomb,mark=none,very thick,red,dashed] file {dat_files/spectral_superres/sines_spectrum.dat};
%\addplot[very thick,violet] file {dat_files/spectral_superres/sines_lowres_long.dat};
%\addplot[black] coordinates {(0,0) (0.5,0)};
%\end{axis}
%\end{tikzpicture} 
%&
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[xmin=-2.5,xmax=23,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,}]
%\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
%\addplot[only marks,very thick,blue] file {dat_files/spectral_superres/sines_samples_long.dat};
%\addplot[black] coordinates {(-10,0) (250,0)};
%\end{axis}
%\end{tikzpicture} 
%\\
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[ticks=none,width=0.6\textwidth, height=0.45\textwidth,xmin=0.1,xmax=0.5] %
%\addplot+[ycomb,mark=none,very thick,red,dashed] file {dat_files/spectral_superres/sines_spectrum.dat};
%\addplot[very thick,violet] file {dat_files/spectral_superres/sines_lowres_long_2.dat};
%\addplot[black] coordinates {(0,0) (0.5,0)};
%\end{axis}
%\end{tikzpicture} 
%&
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[xmin=-2.5,xmax=43,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,}]
%\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
%\addplot[only marks,very thick,blue] file {dat_files/spectral_superres/sines_samples_long_2.dat};
%\addplot[black] coordinates {(-10,0) (100,0)};
%\end{axis}
%\end{tikzpicture} 
%\\
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[ticks=none,xmin=0.1,xmax=0.5,width=0.6\textwidth, height=0.45\textwidth,ticks=none] 
%\addplot+[ycomb,mark=none,very thick,violet] file {dat_files/spectral_superres/sines_spectrum.dat};
%\addplot[black] coordinates {(0,0) (0.5,0)};
%\end{axis}
%\end{tikzpicture}
%& 
%\begin{tikzpicture}[scale=0.75]
%\begin{axis}[xmin=-2.5,xmax=53,width=0.6\textwidth, height=0.4\textwidth,yticklabels={,,}]
%\addplot[dashed,cyan,thick] file {dat_files/spectral_superres/sines.dat};
%\addplot[only marks,very thick,blue] file {dat_files/spectral_superres/sines_samples_long_3.dat};
%\addplot[black] coordinates {(-10,0) (100,0)};
%\end{axis}
%\end{tikzpicture} 
%\end{tabular}
%\end{center}
%\caption{Periodogram (left) and corresponding samples (right) for different numbers of measurements (increasing downwards). In the limit where $n \times \infty$ the frequencies are completely resolved.}
%\label{fig:spectral_sr_formulation}
%\end{figure}

